Impact of Device Thermal Performance on 5G mmWave Communication Systems

5G millimeter wave (mmWave) cellular networks have been reported to deliver 1-2 Gbps downlink throughput, via speed-tests. However, these speed-tests capture only a few seconds of throughput and are not representative of sustained throughput over several minutes. We report the first measurements of sustained throughput in three cities, Miami, Chicago, and San Francisco, where we observe throughput throttling due to rising skin temperature of the phone when it is connected to a deployed 5G mmWave base-station (BS). Radio Resource Control (RRC) messaging between the phone and the BS indicates the reduction in the number of aggregated mmWave channels from 4 to 1 followed by a switch to 4G. We corroborate these measurements with infra-red images as the phone heats up. Thus, mmWave throughput will be limited not by network characteristics but by device thermal management.

==> sections/03_relatedwork.tex <==
% \vspace{-1em}
\section{Related Works}
\label{sec:relatedWorks}

\todo{Related Works}
